Make Graph-based Referring Expression Comprehension Great Again through Expression-guided Dynamic Gating and Regression

One common belief is that with complex models and pre-training on large-scale datasets, transformer-based methods for referring expression comprehension (REC) perform much better than existing graph-based methods. We observe that since most graph-based methods adopt an off-the-shelf detector to locate candidate objects (i.e., regions detected by the object detector), they face two challenges that result in subpar performance: (1) the presence of significant noise caused by numerous irrelevant objects during reasoning, and (2) inaccurate localization outcomes attributed to the provided detector. To address these issues, we introduce a plug-and-adapt module guided by sub-expressions, called dynamic gate constraint (DGC), which can adaptively disable irrelevant proposals and their connections in graphs during reasoning. We further introduce an expression-guided regression strategy (EGR) to refine location prediction. Extensive experimental results on the RefCOCO, RefCOCO+, RefCOCOg, Flickr30K, RefClef, and Ref-reasoning datasets demonstrate the effectiveness of the DGC module and the EGR strategy in consistently boosting the performances of various graph-based REC methods. Without any pretaining, the proposed graph-based method achieves better performance than the state-of-the-art (SOTA) transformer-based methods.

==> bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/author1_jcke.jpg}}]
{Jingcheng Ke} received a B.S. degree in Computer Science and Engineering from Southwest Minzu University,
Chengdu, China, in 2014, and an M.S. degree in Computer Science from Shaanxi Normal University, Xian,
China, in 2018. He received his Ph.D.. degree from Institute of Communications Engineering of National Tsing
Hua University (NTHU), Hsinchu, Taiwan, in 2024. His research interests include referring to expression comprehension, diffusion models, and graphing neural networks.

\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/author2_dwang.jpg}}]
{Dele Wang} received a B.S. degree in Electronic Engineering from the School of Optics and Electronics Information, Huazhong University of Science \& Technology, Wuhan, Hubei, China, in 2018, and an M.S. degree in Electrical Engineering from National Tsing Hua University, Hsinchu, Taiwan, in 2023. His research interests include machine learning, computer vision, and image processing.
\end{IEEEbiography}

%\newpage

\vspace{-0.4in}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio] {photos/author3_jcchen.png}}]
	{Jun-Cheng Chen} (Member, IEEE) is now an Associate Research Fellow at the Research Center for Information Technology Innovation (CITI), Academia Sinica. He joined CITI as an Assistant Research Fellow in 2019. He received the B.S. and M.S. degrees advised by Prof. Ja-Ling Wu in Computer Science and Information Engineering from National Taiwan University, Taiwan (R.O.C), in 2004 and 2006, respectively, where he received the Ph.D. degree advised by Prof. Rama Chellappa in Computer Science from University of Maryland, College Park, USA, in 2016. From 2017 to 2019, he was a postdoctoral research fellow at Institute for Advanced Computer Studies of University of Maryland. His research interests include computer vision, machine learning, deep learning, and their applications to biometrics, such as face recognition/facial analytics, activity recognition/detection in the visual surveillance domain, etc. His works have been recognized in prestigious journals and conferences in the field, including PNAS, TBIOM, CVPR, ICCV, ECCV, FG, WACV, etc. He was a recipient of the ACM Multimedia Best Technical Full Paper Award in 2006 and APSIPA ASC Best Paper Award in 2023.

\end{IEEEbiography}

\vspace{-0.4in}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio] {photos/author4_ihjhuo.jpg}}]
	{I-Hong Jhuo} is a senior applied scientist at Microsoft. He is an active participant in the development of innovative technologies for information retrieval and recommendation system while contributing to advances in the fields of computer vision, structured data and machine learning. Recognized by many awards, conducting the design of a top-performing video analytic system in NIST TRECVIDMED at Columbia University and ACM ACM Multimedia Grand Challenge 2012. His research interests include computer vision, information retrieval, and artificial intelligence.


\end{IEEEbiography}


\vspace{-0.4in}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio] {photos/author5_cwlin.jpg}}]
	{Chia-Wen Lin}
	(Fellow, IEEE) received his Ph.D. degree in Electrical Engineering from National Tsing Hua University (NTHU), Hsinchu, Taiwan, in 2000.  
	Dr. Lin is currently a Distinguished Professor with the Department of Electrical Engineering and the Institute of Communications Engineering, NTHU.  His research interests include image/video processing and computer vision.  He has served as a Fellow Evaluation Committee member (2021--2023), BoG Member-at-Large (2022--2024), and Distinguished Lecturer (2018--2019) of IEEE Circuits and Systems Society.   He was Chair of IEEE ICME Steering Committee (2020--2021). He served as TPC Co-Chair of IEEE ICIP 2019, IEEE ICME 2010, and PCS 2022, and General Co-Chair of IEEE VCIP 2018 and PCS 2024.  He received two best paper awards from VCIP 2010 and 2015. He has served as an Associate Editor of \textsc{IEEE Transactions on Image Processing}, \textsc{IEEE Transactions on Circuits and Systems for Video Technology}, \textsc{IEEE Transactions on Multimedia},  \textsc{IEEE Multimedia}, and Neural Networks. 
\end{IEEEbiography}

\vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/author6_yylin.jpg}}]{Yen-Yu Lin} (Senior Member, IEEE) 
received the B.B.A. degree in Information Management, and the M.S. and Ph.D. degrees in Computer Science and Information Engineering from National Taiwan University, Taipei, Taiwan, in 2001, 2003, and 2010, respectively. He is currently a Distinguished Professor with the Department of Computer Science, National Yang Ming Chiao Tung University, Hsinchu, Taiwan. His research interests include computer vision, machine learning, and artificial intelligence. He serves as an Associate Editor of the International Journal of Computer Vision, Computer Vision and Image Understanding, and ACM Computing Surveys.
\end{IEEEbiography}
